A Survey of OH Masers Towards High Mass Protostellar Objects

We present a survey of OH maser emission towards a sample of high mass protostellar objects made using the Nancay and GBT telescopes.OH maser emission was detected towards 63 objects with 36 new detections. There are 56 star-forming regions and 7 OH/IR candidates. There is no evidence that sources with OH masers have a different range of luminosities from the non-maser sources. The results of this survey are compared with previous water and class II methanol maser observations of the same objects. Some of the detected sources are only associated with OH masers and some sources are only associated with the 1720 MHz OH maser line. The velocity range of the maser emission suggests that the water maser sources may be divided into two groups. The detection rates and velocity range of the OH and Class II methanol masers support the idea that there is a spatial association of the OH and Class II methanol masers. The sources span a wide range in R, the ratio of the methanol maser peak flux to OH 1665 MHz maser peak flux, however there are only a few sources with intermediate values of R, 8<R<32, which has characterised previous samples. Sources which have masers of any species, OH, water or methanol, have redder [100um-12um] IRAS colours than those without masers. However, there is no evidence for different maser species tracing different stages in the evolution of these young high mass sources. Previous observations which have shown that the OH maser emission from similar sources traces the circumstellar disks around the objects. This combined with the sensitivity of the OH emission to the magnetic field, make the newly detected sources interesting candidates for future follow-up at high angular resolution.

==> 6280f17.tex <==
%auto-ignore
%\chapter{}
 %\begin{center}
\begin{figure*}
  \caption{The 9-point maps of the maser intensity integrated over the
    velocity range of each maser component detected by the GBT
    observations. The axes show RA and Dec offset in arcminutes from
    the IRAS position. The contours levels run from 10\% to 90 \% (in
    20\% steps) of the peak flux given in Table~\ref{tab:OHmaserRes}.}
  \label{fig:GBT-map}
%%========================================================================%%
 \clearpage
\resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fsa1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsb1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsc1.eps}
   \includegraphics[angle=-90,width=7cm]{6280fsd1.eps}
 }
%%========================================================================%%
 \newline
  \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fse1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsf1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsg1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsh1.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fsi1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsj1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsk1.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsl1.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsm1.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsn1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fso1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsp1.eps}
 }
\end{figure*}
%%========================================================================%%
\newpage
\begin{figure*}
 \resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fsq1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsr1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fss1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fst1.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fsu1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsv1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsw1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsx1.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fsy1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsz1.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsa2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsb2.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsc2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsd2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fse2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsf2.eps}
}
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsg2.eps}
   \includegraphics[angle=-90,width=7cm]{6280fsh2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsi2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsj2.eps}
 }
\end{figure*}
%%========================================================================%%
%\newpage
\begin{figure*}
 \resizebox{\hsize}{!}{
   \includegraphics[angle=-90,width=7cm]{6280fsk2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsl2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsm2.eps}
   \includegraphics[angle=-90,width=7cm]{6280fsn2.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fso2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsp2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsq2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsr2.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fss2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fst2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsu2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsv2.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsw2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsx2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsy2.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsz2.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsa3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsb3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsc3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsd3.eps}
 }
 \end{figure*}
%%========================================================================%%
 \begin{figure*}
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fse3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsf3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsg3.eps}
   \includegraphics[angle=-90,width=7cm]{6280fsh3.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsi3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsj3.eps}
\includegraphics[angle=-90,width=7cm]{6280fsk3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsl3.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsm3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsn3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fso3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsp3.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsq3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsr3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fss3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fst3.eps}
 }
%%========================================================================%%
 \resizebox{\hsize}{!}{
 \includegraphics[angle=-90,width=7cm]{6280fsu3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsv3.eps}
 \includegraphics[angle=-90,width=7cm]{6280fsw3.eps}
  \includegraphics[angle=-90,width=7cm]{6280fsx3.eps}
 }
 \end{figure*}
%%========================================================================%%
 % \end{center}


==> 6280f18.tex <==
%auto-ignore
%\twocolumn
\begin{center}
\begin{figure*}
 \caption{Same as Figure~\ref{fig:GBT-map} but for OH maser sources offset from
 the IRAS position by $>$ 2$^{'}$.}
  \label{fig:GBT-map-offset}
%%%========================================================================%%
\resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fea1.eps}
  \includegraphics[angle=-90,width=7cm]{6280feb1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fec1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fed1.eps}
 }
  \end{figure*}
%%%========================================================================%%
\begin{figure*}
\resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fee1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fef1.eps}
  \includegraphics[angle=-90,width=7cm]{6280feg1.eps}
  \includegraphics[angle=-90,width=7cm]{6280feh1.eps}
 }
 \end{figure*}
%%%========================================================================%%
\begin{figure*}
\resizebox{\hsize}{!}{
  \includegraphics[angle=-90,width=7cm]{6280fei1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fej1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fek1.eps}
  \includegraphics[angle=-90,width=7cm]{6280fel1.eps}
 }
  \end{figure*}
%%%========================================================================%%
\end{center}
%%%========================================================================%%


==> 6280f19.tex <==
%auto-ignore
\onecolumn
\begin{center}
\begin{figure*}
 \caption{The spectra of each OH maser line detected by GBT and \nancay\
observations. The sources names are given at the top of each group
of spectra. The intensities are in Jy.}
   \label{fig:spectra}
  \includegraphics[angle=-90,width=16cm]{6280fna1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnb1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnc1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnd1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fne1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnf1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fng1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnh1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fni1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnj1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnk1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnl1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnm1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnn1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fno1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnp1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnq1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnr1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fns1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnt1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnu1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnv1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnw1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnx1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fny1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnz1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fna2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnb2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnc2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnd2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fne2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnf2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fng2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnh2.eps}
\end{figure*}
%%========================================================================%%
 \newpage
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fni2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnj2.eps}
\end{figure*}
%%========================================================================%%
 \newpage
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnk2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnl2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnm2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnn2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fno2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnp2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fnq2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnr2.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fns2.eps}
  \includegraphics[angle=-90,width=16cm]{6280fnt2.eps}
\end{figure*}
%%========================================================================%%
  \end{center}
%\end{landscape}


==> 6280f20.tex <==
%auto-ignore
 \begin{center}
\begin{figure*}
  \caption{Same as Figure~\ref{fig:spectra} but for sources with
maser emission offset from the IRAS position by $>$ 2$^{'}$.}
  \label{fig:spectra-offset}
  \includegraphics[angle=-90,width=16cm]{6280fwa1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fwb1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fwc1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fwd1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fwe1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fwf1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fwg1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fwh1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fwi1.eps}
\end{figure*}
%%========================================================================%%
\begin{figure*}
  \includegraphics[angle=-90,width=16cm]{6280fwj1.eps}
  \includegraphics[angle=-90,width=16cm]{6280fwk1.eps}
\end{figure*}
%%========================================================================%%
\end{center}

